GaitMPL: Gait Recognition with Memory-Augmented Progressive Learning

Gait recognition aims at identifying the pedestrians at a long distance by their biometric gait patterns. It is inherently challenging due to the various covariates and the properties of silhouettes (textureless and colorless), which result in two kinds of pair-wise hard samples: the same pedestrian could have distinct silhouettes (intra-class diversity) and different pedestrians could have similar silhouettes (inter-class similarity). In this work, we propose to solve the hard sample issue with a Memory-augmented Progressive Learning network (GaitMPL), including Dynamic Reweighting Progressive Learning module (DRPL) and Global Structure-Aligned Memory bank (GSAM). Specifically, DRPL reduces the learning difficulty of hard samples by easy-to-hard progressive learning. GSAM further augments DRPL with a structure-aligned memory mechanism, which maintains and models the feature distribution of each ID. Experiments on two commonly used datasets, CASIA-B and OU-MVLP, demonstrate the effectiveness of GaitMPL. On CASIA-B, we achieve the state-of-the-art performance, i.e., 88.0% on the most challenging condition (Clothing) and 93.3% on the average condition, which outperforms the other methods by at least 3.8% and 1.4%, respectively.

==> fig/memory.tex <==
\begin{figure}[t]
    \begin{center}
       \includegraphics[width=8.5cm]{img/memory_bank.pdf}
    \end{center}
    \caption{The illustration of GSAM, which models the ID-level features for each ID. \romannumeral1) The memory elements of GSAM are the centroid features of each ID. $\otimes$ denotes the aggregation operator covering various covariates. \romannumeral2) IDs present/absent in the current batch are both updated in GSAM according to corresponding strategies.}
    \label{fig:memory}
 \end{figure}

==> fig/momentum.tex <==
\begin{figure}[t]
    \begin{center}
       \includegraphics[width=0.8\linewidth]{./img/momentum.pdf}
    \end{center}
    \caption{The effect of the momentum $\alpha$ and $\beta$ in GSAM. Too large or too small momentum will decrease the performance.}
    \label{fig:ab_momentum}
 \end{figure}

==> tab/ab_memory.tex <==



\begin{table}[]
      \centering
      \begin{tabular}{l|cccc}
            \toprule
      Method           & NM   & BG   & CL   & AVG  \\
      \hline
      GaitSet          & 94.2 & 88.2 & 71.8 & 84.7 \\
      GaitSet+ D       & 95.3 & 88.8 & 73.7 & 85.9 \\
      GaitSet+ D + G   & 95.6 & 88.8 & 80.9 & 88.4 \\ \hline
      GaitPart         & 95.4 & 91.3 & 82.3 & 89.6 \\
      GaitPart +  D    & 95.5 & 91.3 & 82.8 & 89.9 \\
      GaitPart + D + G & 95.7 & 91.9 & 83.8 & 90.5 \\ \hline
      MT3D             & 96.6 & 93.0 & 82.2 & 90.6 \\
      MT3D + D         & 95.1 & 92.5 & 86.8 & 91.5 \\
      MT3D + D + G     & 95.5 & 92.9 & 87.9 & 92.2 \\ 
      \bottomrule
      \end{tabular}
      \end{table}

==> tab/ab_reweighting.tex <==
\begin{table}[]
    \centering
    \caption{Performance on Different sampling reweighting Strategy in DRPL}
    \begin{tabular}{l|r|r|r|r}
    \toprule
    Strategy            & \multicolumn{1}{c|}{NM} & \multicolumn{1}{c|}{BG} & \multicolumn{1}{c|}{CL}     & \multicolumn{1}{c}{AVG}    \\ \midrule
    Baseline    & 94.2                 & 88.2                  & 71.8                      & \multicolumn{1}{c}{84.7} \\ \hline
    Easier Sampler      & 94.4                 & 87.6                  & 73.5                        & 85.1                      \\ \hline
    MinMax              & 94.3                  & 87.3                  & 75.2                  & 85.6                      \\ \hline
    Dynamic Polynomial  & 94.4                    & 88.1                  & 74.8                      & 85.7                      \\ \hline
    Exponential         & 94.6                  & 87.8                  & \multicolumn{1}{l|}{72.8} & 85.1                      \\ \hline
    Dynamic Exponential & 95.3                  & 88.8                  & 73.7                      & \multicolumn{1}{c}{85.9}  \\ \bottomrule
    \end{tabular}
    \end{table}








==> tab/structure.tex <==
\begin{table}[t!]
   \caption{Detail structure of our encoder network.}
   \label{tab:structure}
   \begin{center}
       % \resizebox{\textwidth}{!}{
       \scalebox{0.7}{
           \begin{tabular}{lll}
               \hline
               \multicolumn{1}{l|}{\textbf{Operation}} & \multicolumn{1}{l|}{\textbf{Details}}                                                               & \textbf{Output shape}               \\ \hline
               \multicolumn{3}{c}{\textbf{BackBone}}                                                                                                                                               \\ \hline
               \multicolumn{1}{l|}{Input}              & \multicolumn{1}{l|}{$T \times C \times H \times W$}                                                 & $30 \times 1 \times 64 \times 44$   \\
               \multicolumn{1}{l|}{Block 1}            & \multicolumn{1}{l|}{\texttt{Conv2D} [1, 5, 5, 32], padding=2 - \texttt{BN} - \texttt{LeakyReLU}}    & $30 \times 32 \times 64 \times 44$  \\
               \multicolumn{1}{l|}{Block 2}            & \multicolumn{1}{l|}{\texttt{Conv2D} [32, 3, 3, 32], padding=1 - \texttt{BN} - \texttt{LeakyReLU}}   & $30 \times 32 \times 64 \times 44$  \\
               \multicolumn{1}{l|}{Downsample}         & \multicolumn{1}{l|}{\texttt{MaxPool2D} [2, 2]}                                                      & $30 \times 64 \times 32 \times 22$  \\
               \multicolumn{1}{l|}{Block 3}            & \multicolumn{1}{l|}{\texttt{Conv2D} [32, 3, 3, 64], padding=1 - \texttt{BN} - \texttt{LeakyReLU}}   & $30 \times 64 \times 32 \times 22$  \\
               \multicolumn{1}{l|}{Block 4}            & \multicolumn{1}{l|}{\texttt{Conv2D} [64, 3, 3, 64], padding=1 - \texttt{BN} - \texttt{LeakyReLU}}   & $30 \times 64 \times 32 \times 22$  \\
               \multicolumn{1}{l|}{Downsample}         & \multicolumn{1}{l|}{\texttt{MaxPool2D} [2, 2]}                                                      & $30 \times 64 \times 16 \times 11$  \\
               \multicolumn{1}{l|}{Block 5}            & \multicolumn{1}{l|}{\texttt{Conv2D} [64, 3, 3, 128], padding=1 - \texttt{BN} - \texttt{LeakyReLU}}  & $30 \times 128 \times 16 \times 11$ \\
               \multicolumn{1}{l|}{Block 6}            & \multicolumn{1}{l|}{\texttt{Conv2D} [128, 3, 3, 128], padding=1 - \texttt{BN} - \texttt{LeakyReLU}} & $30 \times 128 \times 16 \times 11$ \\ \hline
               \multicolumn{3}{c}{\textbf{Temporal Module}}                                                                                                                                        \\ \hline
               \multicolumn{1}{l|}{Reshape}            & \multicolumn{1}{l|}{$T \times C \times H \times W \rightarrow (H*W) \times C \times T$}             & $(16*11) \times 128 \times 30$      \\
               \multicolumn{1}{l|}{Temporal Branch T1} & \multicolumn{1}{l|}{\texttt{Conv1D} [128, 3, 128], padding=1, dilation=1}                           & $(16*11) \times 128 \times 30$      \\
               \multicolumn{1}{l|}{Temporal Branch T2} & \multicolumn{1}{l|}{\texttt{Conv1D} [128, 3, 128], padding=2, dilation=2}                           & $(16*11) \times 128 \times 30$      \\
               \multicolumn{1}{l|}{Temporal Branch T3}          & \multicolumn{1}{l|}{\texttt{Conv1D} [128, 3, 128], padding=4, dilation=4}                           & $(16*11) \times 128 \times 30$      \\
               \multicolumn{1}{l|}{Concat(T1, T2, T3)} & \multicolumn{1}{l|}{Along axis 1}                                                                   & $(16*11) \times 384 \times 30$      \\
               \multicolumn{1}{l|}{Downsample}         & \multicolumn{1}{l|}{\texttt{GlobalMaxPool1D}, kernel size=30}                                       & $(16*11) \times 384$                \\ \hline
               \multicolumn{3}{c}{\textbf{Aggregation Module}}                                                                                                                                             \\ \hline
               \multicolumn{1}{l|}{Reshape}            & \multicolumn{1}{l|}{$(H*W) \times C \rightarrow C \times H \times W$}                               & $384 \times 16 \times 11$           \\
               \multicolumn{1}{l|}{Pooling Branch P1}  & \multicolumn{1}{l|}{\texttt{GlobalMeanPool1D}, kernel size=11}                                      & $384 \times 16$                     \\
               \multicolumn{1}{l|}{Pooling Branch P2}  & \multicolumn{1}{l|}{\texttt{GlobalMaxPool1D}, kernel size=11}                                       & $384 \times 16$                     \\
               \multicolumn{1}{l|}{Add(P1, P2)}        & \multicolumn{1}{l|}{\texttt{ElementwiseAdd}}                                                        & $384 \times 16$                     \\
               \multicolumn{1}{l|}{Seprate FC}         & \multicolumn{1}{l|}{For each bin, \texttt{FC} [384, 256]. Note they don't share params.}            & $256 \times 16$                     \\ \hline
           \end{tabular}
       }
   \end{center}

\end{table}
